Choosability with union separation

List coloring generalizes graph coloring by requiring the color of a vertex to be selected from a list of colors specific to that vertex. One refinement of list coloring, called choosability with separation, requires that the intersection of adjacent lists is sufficiently small. We introduce a new refinement, called choosability with union separation, where we require that the union of adjacent lists is sufficiently large. For $t \geq k$, a $(k,t)$-list assignment is a list assignment $L$ where $|L(v)| \geq k$ for all vertices $v$ and $|L(u)\cup L(v)| \geq t$ for all edges $uv$. A graph is $(k,t)$-choosable if there is a proper coloring for every $(k,t)$-list assignment. We explore this concept through examples of graphs that are not $(k,t)$-choosable, demonstrating sparsity conditions that imply a graph is $(k,t)$-choosable, and proving that all planar graphs are $(3,11)$-choosable and $(4,9)$-choosable.

==> figures/book-k02-t02.tex <==
\begin{tikzpicture}[vtx/.style={shape=coordinate}]
	\node[vtx] (v0) at (-0.5000,1.0000) {};
	\node[vtx] (v1) at (0.5000,1.0000) {};
	\node[vtx] (v2) at (-0.5000,0.0000) {};
	\node[vtx] (v3) at (0.5000,0.0000) {};
	\draw (v0) -- (v1);
	\draw (v0) -- (v2);
	\draw (v0) -- (v3);
	\draw (v1) -- (v2);
	\draw (v1) -- (v3);
	\foreach \p in {v0,v1,v2,v3}
	{
		\blackvertex{\p}
	}
\end{tikzpicture}


==> figures/book02.tex <==
\begin{tikzpicture}[vtx/.style={shape=coordinate}]
	\node[vtx] (v0) at (0.0000,0.0000) {};
	\node[vtx] (v1) at (0.0000,2.0000) {};
	\node[vtx] (v2) at (1.0000,1.0000) {};
	\node[vtx] (v3) at (2.0000,1.0000) {};
	\draw (v0) -- (v1);
	\draw (v0) -- (v2);
	\draw (v0) -- (v3);
	\draw (v1) -- (v2);
	\draw (v1) -- (v3);
	\foreach \p in {v0,v1,v2,v3}
	{
		\blackvertex{\p}
	}
\end{tikzpicture}

